Channel Merging: Preserving Specialization for Merged Experts

Lately, the practice of utilizing task-specific fine-tuning has been implemented to improve the performance of large language models (LLM) in subsequent tasks. Through the integration of diverse LLMs, the overall competency of LLMs is significantly boosted. Nevertheless, traditional ensemble methods are notably memory-intensive, necessitating the simultaneous loading of all specialized models into GPU memory. To address the inefficiency, model merging strategies have emerged, merging all LLMs into one model to reduce the memory footprint during inference. Despite these advances, model merging often leads to parameter conflicts and performance decline as the number of experts increases. Previous methods to mitigate these conflicts include post-pruning and partial merging. However, both approaches have limitations, particularly in terms of performance and storage efficiency when merged experts increase. To address these challenges, we introduce Channel Merging, a novel strategy designed to minimize parameter conflicts while enhancing storage efficiency. This method clusters and merges channel parameters based on their similarity to form several groups offline. By ensuring that only highly similar parameters are merged within each group, it significantly reduces parameter conflicts. During inference, we can instantly look up the expert parameters from the merged groups, preserving specialized knowledge. Our experiments demonstrate that Channel Merging consistently delivers high performance, matching unmerged models in tasks like English and Chinese reasoning, mathematical reasoning, and code generation. Moreover, it obtains results comparable to model ensemble with just 53% parameters when used with a task-specific router.

==> checklist.tex <==
\section{Paper Checklist}
\begin{enumerate}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced: Yes
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: Yes
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: Yes
\item Does this paper make theoretical contributions? No
\item Does this paper rely on one or more datasets? Yes
\item A motivation is given for why the experiments are conducted on the selected datasets: yes
\item All novel datasets introduced in this paper are included in a data appendix. NA
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. NA
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. Yes
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. Yes
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. NA
\item Does this paper include computational experiments? Yes
\item Any code required for pre-processing data is included in the appendix. NA
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from: Yes
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results: Yes
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks: Yes
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics: Yes
\item This paper states the number of algorithm runs used to compute each reported result: Yes
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information: Yes
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank): No
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments: NA
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting: NA
\end{enumerate}
